Swift X-ray Observations of Classical Novae

The new gamma-ray burst mission Swift has obtained pointed observations of several classical novae in outburst. We analyzed all the observations of classical novae from the Swift archive up to 30 June, 2006. We analyzed usable observations of 12 classical novae and found 4 non-detections, 3 weak sources and 5 strong sources. This includes detections of 2 novae exhibiting spectra resembling those of Super Soft X-ray binary Source spectra (SSS) implying ongoing nuclear burning on the white dwarf surface. With these new Swift data, we add to the growing statistics of the X-ray duration and characteristics of classical novae.

==> figs3to4.tex <==
\begin{figure*}
\resizebox{\hsize}{!}{\includegraphics{f03}}
\caption{\label{firstphot}Illustration of extraction of counts.
{\bf Left panel}: We show the recorded photon positions and mark the source
extraction region with dark shading and the background extraction region
(annulus with inner radius 10\,pixels and outer radius 100\,pixels) with
light shading. The count rate, detection likelihood, and the model
parameters $S$ and $B$ determined from Eq.~\ref{model} are given in the
upper left.
Observation date, number of source- and background counts per detect cell,
and exposure time are given in the upper right. The percentage of source counts
that reside within 25\,percent area (radius 5\,pixels) is given to the right
of the source extraction region to demonstrate the concentration
of counts towards the center of the source extraction region.
{\bf Right panel}: Spectral information of
the source (black) and background (scaled to the area of the source extraction
region; light shadings). The likelihood for the
background spectrum being softer than the source spectrum is estimated by
drawing 1000 random sample spectra, with the same number of
source counts (72), out
of the background ($4\times 99=396$ counts) and
counting the number of cases where the median energy for each sample
spectrum is lower than that of the source spectrum. Much different values
than 50\,percent are a soft criterion for a source detection.}
\end{figure*}

\begin{figure*}
\resizebox{\hsize}{!}{\includegraphics{f04}}
\caption{\label{lastphot}Same as Fig.~\ref{firstphot} for V723\,Cas (top)
and V4743\,Sgr (bottom). While the count rates are similar,
the observed spectra are very different.}
\end{figure*}


